Optimisation Strategies for Ensuring Fairness in Machine Learning: With and Without Demographics

Ensuring fairness has emerged as one of the primary concerns in AI and its related algorithms. Over time, the field of machine learning fairness has evolved to address these issues. This paper provides an extensive overview of this field and introduces two formal frameworks to tackle open questions in machine learning fairness. In one framework, operator-valued optimisation and min-max objectives are employed to address unfairness in time-series problems. This approach showcases state-of-the-art performance on the notorious COMPAS benchmark dataset, demonstrating its effectiveness in real-world scenarios. In the second framework, the challenge of lacking sensitive attributes, such as gender and race, in commonly used datasets is addressed. This issue is particularly pressing because existing algorithms in this field predominantly rely on the availability or estimations of such attributes to assess and mitigate unfairness. Here, a framework for a group-blind bias-repair is introduced, aiming to mitigate bias without relying on sensitive attributes. The efficacy of this approach is showcased through analyses conducted on the Adult Census Income dataset. Additionally, detailed algorithmic analyses for both frameworks are provided, accompanied by convergence guarantees, ensuring the robustness and reliability of the proposed methodologies.

==> optimisation/arxiv.tex <==
\paragraph{Learning of Linear Dynamical Systems as a Non-Commutative Polynomial Optimisation Problem}
There has been much recent progress in time series forecasting and estimation of system matrices of linear dynamical systems. 
We present an approach to both problems based on an asymptotically convergent hierarchy of convexifications of a certain non-convex operator-valued problem, which is known as non-commutative polynomial optimisation. We present promising computational results,
including a comparison with methods implemented in Matlab System Identification Toolbox.
This is published in the IEEE Transactions on Automatic Control \citep{zhou2023learning}.

\paragraph{Fairness in Forecasting of Observations of Linear Dynamical Systems}
In machine learning, training data often capture the behaviour of multiple subgroups of some underlying human population.
This behaviour can often be modelled as observations of an unknown dynamical system with an unobserved state.
When the training data for the subgroups are not controlled carefully,  however, under-representation bias arises.
To counter under-representation bias, we introduce two natural notions of fairness in time-series forecasting problems: subgroup fairness and instantaneous fairness.
These notions extend predictive parity to the learning of dynamical systems.
We also show globally convergent methods for the fairness-constrained learning problems using hierarchies of convexifications of non-commutative polynomial optimisation problems. 
We also show that by exploiting sparsity in the convexifications, we can reduce the run time of our methods considerably.
Our empirical results on a biased dataset motivated by insurance applications and the well-known COMPAS dataset demonstrate the efficacy of our methods.
This is published in the Journal of Artificial Intelligence Research \citep{zhou2023fairness}, with a preliminary version presented in the AAAI Conference on Artificial Intelligence \citep{zhou2021fairness}.

\paragraph{Group-Blind Optimal Transport to Group Parity and Its Constrained Variants}
Fairness plays a pivotal role in the realm of machine learning, particularly when it comes to addressing groups categorised by sensitive attributes, e.g., gender, race. 
Prevailing algorithms in fair learning predominantly hinge on accessibility or estimations of these sensitive attributes.
We design a single group-blind projection map that aligns the feature distributions of both groups in the source data, achieving (demographic) group parity, without requiring values of the sensitive attribute for individual samples in the computation of the map, as well as its use.
Instead, our approach utilises the feature distributions of the privileged and unprivileged groups in a boarder population and the essential assumption that the source data are unbiased representation of the population.
We present numerical results on synthetic data and the well-known Adult Census Income dataset. This is under review  and can be found on arXiv \citep{zhou2023group}.



\paragraph{Subgroup Fairness in Two-Sided Markets}
It is well known that two-sided markets are unfair in a number of ways. 
For example, female drivers on ride-hailing platforms earn less than their male colleagues per mile driven.
Similar observations have been made for other minority subgroups in other two-sided markets. 
Here, we suggest a novel market-clearing mechanism for two-sided markets, which promotes equalisation of the pay per hour worked across multiple subgroups, as well as within each subgroup.
In the process, we introduce a novel notion of subgroup fairness (which we call Inter-fairness), 
which can be combined with other notions of fairness within each subgroup (called Intra-fairness), 
and the utility for the customers (Customer-Care) in the objective of the market-clearing problem. 
Although the novel non-linear terms in the objective complicate market clearing by making the problem non-convex, 
we show that a certain non-convex augmented Lagrangian relaxation can be approximated to any precision in time polynomial in the number of market participants using semidefinite programming, thanks to its ``hidden convexity''.
This makes it possible to implement the market-clearing mechanism efficiently.
On the example of a driver-ride assignment system, we demonstrate the efficacy and scalability of the approach and trade-offs between Inter- and Intra-fairness. This is published in the PLOS ONE \citep{zhou2023subgroup}.



\subsection{Dual}

Now if we look at the dual problem, it is also an SDP.

\begin{definition}[The dual cones]{\cite{burgdorf2016optimization}, Remark~1.64.}\label{defin:dual cones}
%We define the dual cone $\left(\Theta_{2d}\right)^{\vee}$ to consist of symmetric linear functionals which are nonnegative on $\Theta_{2d}$ and zero on commutators.
If given $\mathbf{g}\subseteq\Sym\mathbb{R}[\mathbf{X}]$, we define the dual cone $\left(\Theta_{2d}(\mathbf{g})\right)^{\vee}$ to consist of symmetric linear functionals which are nonnegative on $\Theta_{2d}(\mathbf{g})$ and zero on commutators.
%give a constrained dual cone. 
Using the Hankel matrix $M_k$, the dual cone can also be rewritten as a set of LMI.
\begin{eqnarray*}
%\left(\Theta_{2d}\right)^{\vee}:&=&\{L:\mathbb{R}[\mathbf{X}]_{2d}\to\mathbb{R}\ \;|\; L \textrm{ linear}, L(p)=L(p^{\dag}),L(p)\geq 0, \forall p\in \Theta_{2d}\},\nonumber\\
%&\cong&\{M_k\;|\;M_k\succcurlyeq 0, (M_k)_{u,v}=(M_k)_{w,z},\; \forall u^{\dag}v \stackrel{\cyc}{\sim} w^{\dag}z \}.\\
\left(\Theta_{2d}(\mathbf{g})\right)^{\vee}:&=&\{L:\mathbb{R}[\mathbf{X}]_{2d}\to\mathbb{R}\ \;|\; L \textrm{ linear}, L(p)=L(p^{\dag}),L(p)\geq 0, \forall p\in \Theta_{2d}(\mathbf{g})\}.\nonumber\\
&\cong&\{M_k\;|\;M_k\succcurlyeq 0; M_{k_i}\succcurlyeq 0,\;\forall q\in Q; (M_k)_{u,v}=(M_k)_{w,z},\; \forall u^{\dag}v \stackrel{\cyc}{\sim} w^{\dag}z \}.
\end{eqnarray*}
\end{definition}


%Suppose $M_k$ is an extension of another Hankel matrix $H_{\check{L}}$ with $\rk H_{\check{L}}=\rk M_k$, we say that $M_k$ is flat over $H_{\check{L}}$.
%Further, suppose their corresponding linear functionals being $L:\mathbb{R}[\mathbf{X}]_{2d}\to\mathbb{R}$ and $\check{L}:\mathbb{R}[\mathbf{X}]_{2k-2\delta}\to\mathbb{R}$, we say that $L$ is $\delta$-flat.
% \begin{remark}[]{} 
% \label{cor:transfer to Hankel}
% Given two polynomials $f,g\in\mathbb{R}[\mathbf{X}]$ and $f=\sum_{u} f_u u$, $g=\sum_{\nu} g_{\nu} \nu$.
% Following the definition of the Hankel matrix $M_k$, we have that 
% \begin{equation}
% L(f^{\dag} g)=\sum_{u,\nu}f_u g_{\nu} L(u^{\dag}\nu)=\sum_{u,\nu}f_u g_{\nu} (M_k)_{u,\nu}=\overrightarrow{f}' M_k\overrightarrow{g}.
% \end{equation}
%where $\overrightarrow{p},\overrightarrow{q}$ are vectors consisting of all coefficients $p_{u}$ of $p$ and $q_{\nu}$ of $q$.
% \end{remark}
\begin{lemma}[Positivity of $L$ is equivalent to the positive semidefinitness of $M_k$]{\cite{burgdorf2016optimization}, Lemma~1.44.}
According to the definition, $L$ is nonnegative on $\mathbf{M}_{Q,2k}$. 
Given two polynomials $f,g\in\mathbb{R}[\mathbf{X}]$ and $f=\sum_{u} f_u u$, $g=\sum_{\nu} g_{\nu} \nu$.
Following the definition of the Hankel matrix $M_k$, we have that 
\begin{equation}
L(f^{\dag} g)=\sum_{u,\nu}f_u g_{\nu} L(u^{\dag}\nu)=\sum_{u,\nu}f_u g_{\nu} (M_k)_{u,\nu}=\overrightarrow{f}' M_k\overrightarrow{g}.
\end{equation}
Hence, it is easy to see that
\begin{equation}
M_k\succcurlyeq 0;\; M_{k_i}\succcurlyeq 0,\;\forall q\in Q.
\end{equation}
\end{lemma}
In the tracial cases, $L$ also needs to be zero on commutators, hence $M_k$ is invariant under cyclic equivalence, such that for $u,v,w,z\in [X]_{k}$
\begin{equation}
    (M_k)_{u,v}=(M_k)_{w,z},\; \forall\;u^{\dag}v \stackrel{\cyc}{\sim} w^{\dag}z. 
\end{equation}


To obtain the dual problem of \eqref{trace-NCPO-uncon-sup-Theta}, we conduct the standard Lagrangian duality approach, such that
\begin{eqnarray}
\tr_{\Theta^2}(p)&:=&
\begin{array}{cl}
\sup_{a} & a  \\
\textrm{s.t.} & p-a\in\Theta_{2d}
\end{array} \\
&=&\sup_a \inf_{L\in\left(\Theta_{2d}\right)^{\vee}} \left\{ a + L(p-a) \right\}
\label{equ:cone-transfer} \\
&\leq &\inf_{L\in\left(\Theta_{2d}\right)^{\vee}}\sup_a \left\{ a + L(p-a)\right\} \label{equ:weak duality}\\
&=& \inf_{L\in\left(\Theta_{2d}\right)^{\vee}}\sup_a \left\{a + L(p)-a L(1) \right\}\label{equ:linearity of L}\\
&=& \inf_{L\in\left(\Theta_{2d}\right)^{\vee}}  \left\{ L(p) +\sup_a \{a(1- L(1))\} \right\}\label{equ:inner problem}\\
&=&\begin{array}{cl}
\inf & L(p)  \\
\textrm{s.t.} & L\in\left(\Theta_{2d}\right)^{\vee}\\ & L(1)=1.
\end{array}
=:L_{\Theta^2}(p)
\label{equ:trace-NCPO-dual}
\end{eqnarray}
The equality in \eqref{equ:cone-transfer} uses the Definition~\ref{defin:dual cones} to transfer the cone constraint. The inequality in \eqref{equ:weak duality} utilizes the weak duality, since the variable $a$ is unbounded. The equality in \eqref{equ:linearity of L} is due to the linearity of $L$. Finally, the inner problem in \eqref{equ:inner problem} is bounded only if $L(1)=1$, such that we obatin the dual problem in \eqref{equ:trace-NCPO-dual}.
Note that the same procedures could be applied to \eqref{trace-NCPO-con-sup-Theta} simply by changing $\Theta_{2d}$ to $\Theta_{2d}(\mathbf{g})$, and the resulted formulation is denoted by $L^{k}_{\Theta^2}(p,Q)$.

\begin{theorem}[]{$L_{\Theta^2}(p),L^k_{\Theta^2}(p,Q)$ are SDP.}
\end{theorem}
\begin{proof}
For $L_{\Theta^2}(p)$, we can transfer this problem to the space of Hankel matrix $M_k$.
We first look at the objective function of \eqref{equ:trace-NCPO-dual}.
Since $p\in\Sym\mathbb{R}[\mathbf{X}]_{2d}$, the polynomial $p$ can be expressed by a Gram matrix $G_p$, such that $p=\mathbf{W}^{\dag}_{k} G_p \mathbf{W}_{k}$ and $G_p$ is symmetric.
Using the proof of Lemma~\ref{lem:gram matrix}, we have
\begin{eqnarray*}
L(p)&=&L\left(\sum_{\omega\in \mathbf{W}_{2d}}p_{\omega}( \omega + \omega^{\dag})\right)\\
&=&\sum_{\omega\in \mathbf{W}_{2d}}p_{\omega} L( \omega + \omega^{\dag})\\
&=&\sum_{\omega\in \mathbf{W}_{2d}}p_{\omega}\left( L(u^{\dag}\nu) + L(\nu^{\dag} u)\right)\\
&=&\sum_{\omega\in \mathbf{W}_{2d}}p_{\omega}\left( \overrightarrow{u}' M_k\overrightarrow{\nu} + \overrightarrow{\nu}' M_k\overrightarrow{u}\right)\\
&=&\left\langle M_k,\sum_{\omega\in \mathbf{W}_{2d}}p_{\omega}\left(\overrightarrow{u}\overrightarrow{\nu}'+\overrightarrow{\nu}\overrightarrow{u}'\right)\right\rangle \\
&=& \langle M_k,G_p\rangle 
\end{eqnarray*}
Then, using Definition~\ref{defin:dual cones}, the first constraint $L\in\left(\Theta_{2d}\right)^{\vee}$ is a set of LMI . 
The last constraint $L(1)=1$ is equivalent to $\langle M_k, E_{1,1}\rangle=1$, where $E_{1,1}$ is a matrix with all entries 0 but $1$ in the $(1,1)$-entry. 
Further, $L^{k}_{\Theta^2}(p,Q)$ only differs from $L_{\Theta^2}(p)$ by the dual cone constraint. By reusing Definition~\ref{defin:dual cones}, we know that $L^{k}_{\Theta^2}(p,Q)$ is also a SDP.
\end{proof}

\begin{lemma}[\cite{helton2002positive}, Lemma~2.1]{}\label{lem:gram matrix}
For a polynomial $f\in\Sym\mathbb{R}[\mathbf{X}]_{2d}$, there exist a (non-unique) Gram matrix $G_f$, such that  
\begin{equation*}
f=W_{d}^{\dag}\; G_f\; W_{d},\; G^{\dag}_f=G_f,
\end{equation*}
where $W_{d}$ is a vector consisting all monomials in $\mathbf{W}_{d}$, which is introduced in Definition~\ref{def:monomial_basis_nc}.
\end{lemma}
\begin{proof}
A symmetric polynomial $f\in\Sym\mathbb{R}[\mathbf{X}]_{2d}$ is a weighted sum of symmetrised monomials, such that 
\begin{equation}
f=\sum_{\omega\in \mathbf{W}_{2d}}f_{\omega}( \omega + \omega^{\dag}),\label{equ:sum of symmetrized monomials}
\end{equation}
where $\omega\in \mathbf{W}_{2d}$ could be written as a product of two monomials
\begin{equation*}
\omega=u^{\dag} \nu,
\end{equation*}
with $u,\nu\in\mathbf{W}_d$. 
%\textcolor{red}{Recall from Section~\ref{app:GNS} that}
Let $\overrightarrow{f}$ denote the vector of coefficients of $f\in\mathbb{R}[\mathbf{X}]$.
Monomials $u,\nu$ could also be regarded as a polynomial, with
\begin{equation*}
u=\overrightarrow{u}'W_d,\; \nu=\overrightarrow{\nu}'W_d.
\end{equation*}
Since $\omega=\mathbf{W}^{\dag}_d \overrightarrow{u}\overrightarrow{\nu}'W_d$ and $\omega^{\dag}=\mathbf{W}^{\dag}_d \overrightarrow{\nu}\overrightarrow{u}'W_d$,
we show that the symmetrised monomial $\omega+\omega^{\dag}$ could be associated with a symmetric Gram matrix, such that 
\begin{equation}
\omega + \omega^{\dag}=W^{\dag}_d \left(\overrightarrow{u}\overrightarrow{\nu}'+\overrightarrow{\nu}\overrightarrow{u}'\right)W_d.
\label{equ:a symmetrized monomial}
\end{equation}
Substituting \eqref{equ:a symmetrized monomial} for \eqref{equ:sum of symmetrized monomials}, we then obtain a Gram matrix $G_f$ of $f$ as follows:
\begin{equation*}
G_f=\sum_{\omega\in \mathbf{W}_{2d}}p_{\omega}\left(\overrightarrow{u}\overrightarrow{\nu}'+\overrightarrow{\nu}\overrightarrow{u}'\right).
\end{equation*}
Using the fact that the weighted sum of symmetric matrices is also symmetric, we complete the proof.
\end{proof}

\section{The exploiting correlative sparsity variant}
\label{sec:sparsitytheory}

There is much room of sparsity exploiting in the interest of significant reduction in runtime. Here, we give a brief summary of correlative sparsity exploiting trace optimisation, and we refer readers to \cite{klep2021sparse} for more details and to \cite{wang2021exploiting} for term sparsity exploiting variant.

The index set of the tuple $\mathbf{X}\in\mathbb{S}^n$ is $I=\{1,2,\dots,n\}$. Suppose there is a partition such that $I_1,I_2,\dots, I_r\subseteq I$ and $\bigcup^r_{i=1} I_i=I$. 
Let $X(I_i)\subset X$ denote the set of variables $X_j$ whose indices belong to $I_i$.
Given a sparse objective function $p\in\Sym\mathbb{R}[\mathbf{X}]$, we assume that $p$ can be decomposed as
\begin{equation*}
p=p_1 + p_2 + \cdots + p_r,
\end{equation*}
where $p_i\in\Sym\mathbb{R}[X(I_i)]$.
With the assumptions of boundedness of each subset $X(I_i)$ and running intersection property, cf. Assumptions~2,3 and 2.4 in \cite{klep2021sparse}, we obtain the sparse trace minimization formulations:
\begin{definition}[\cite{klep2021sparse}]{Sparse semialgebraic sets.}
Given a subset of polynomials $Q\subseteq\Sym\mathbb{R}[\mathbf{X}]$ and the sparse version of $\mathscr{D}^{\spa}_Q$ is defined as
\begin{eqnarray*}
\mathscr{D}^{\spa}_Q:=\mathscr{D}_Q\bigcap \left\{\mathbf{X}\in\mathbb{S}^n \;|\;\exists N\in\mathbb{R}_{+}: N-\sum_{j\in I_i} X^2_j\succcurlyeq 0,i=1,2,\dots,r\right\}.
\end{eqnarray*}
\end{definition}
\begin{definition}[\cite{klep2021sparse}]{Sparse cyclic quadratic modules.}
Given a subset of polynomials $Q\subseteq\Sym\mathbb{R}[\mathbf{X}]$ and the sparse version of $\mathscr{D}^{\spa}_Q$. We define
\begin{eqnarray*}
\Theta^{\spa}_{Q,2k}&:=&\Theta^{1}_{Q,2k}+\Theta^{2}_{Q,2k}+\cdots+\Theta^{r}_{Q,2k},\\
\Theta^{i}_{Q,2k}&:=&\left\{f\in\Sym\mathbb{R}[X(I_i)] \;|\; \exists g\in \mathbf{M}^{i}_{Q,2k}: f\stackrel{\cyc}{\sim} g \right\}.
\end{eqnarray*}
For unconstrained cases, we can drop the $Q$ in subscriptions, i.e., $Q=\varnothing$.
\end{definition}
Then, by replacing $\Theta^2_{2k_1}$ in \eqref{trace-NCPO-uncon-sup-Theta} with $\Theta^{\spa}_{2k_1}$, we get the sparse formulation $\tr_{\Theta^{\spa}}(p)$. Similarly, we get the sparse formulation for constrained case $\tr^{k_2}_{\Theta^{\spa}}(p,Q)$ by substituting $\Theta^2_{Q,2k_2}$ in \eqref{trace-NCPO-con-sup-Theta} with $\Theta^{\spa}_{Q,2k_2}$.

Alongside with sparse trace minimization, one can also exploit the constant trace property for SDP relaxations, see \cite{mai2021constant}.


%\tr^{k_2}_{\Theta^2}(p,Q)&:=\sup\{a\;|\;f-a\in\Theta^2_{Q,2k_2}\} \leq\tr^{\II}_{\min}(Q,p)\leq\tr_{\min}(Q,p),\label{trace-NCPO-con-sup-Theta}




%\section{Exploiting Sparsity}

The computational load of non-commutative polynomial optimisation (Section~\ref{sec:ncpop}), can be lifted via  sparsity exploiting variants \citep{klep2021sparse,wang2021tssos}.


\begin{assumption}[Running Intersection Property]
With $\mathbf{x}=(x_1,\dots,x_n)$, let $I_0:=\{1,\dots,n\}$ be the union $\cup_{k=1}^{\ell}$ of $\ell$ subsets $I_{k}$, $k=1,\dots,\ell$ (with possible overlaps). Let $\mathbb{R}[\mathbf{x}(I_k)]$ denote the ring of polynomials in the subset of variables $\mathbf{x}(I_k)=\{x_i:i\in I_k\}$ and so $\mathbb{R}[\mathbf{x}(I_0)]=\mathbb{R}[\mathbf{x}]$.
Let $\mathbb{K}$ be as in Definition~\ref{def:semi-algebraic}, with $(g_j)_{j=1}^{m}\subset\mathbb{R}[\mathbf{x}]$. The index set $J=\{1,\dots,m\}$ is partitioned into $\ell$ disjoint sets $J_k$, $k=1,\dots,\ell$, and the collections $\{I_k\}$ and $\{J_k\}$ satisfy:
\end{assumption}

\section{Minimiser Extraction}


\begin{definition}[Sums of Hermitian Squares (sohs)]\label{def:sohs}
% An nc polynomial $f\in\mathbb{R}[\mathbf{X}]$ is a sum of Hermitian squares if can be written as
% \begin{equation*}
% f=\sum_{i} f_i^{\dag}f_i,
% \end{equation*}
% for some finite family of nc polynomials $f_i\in\mathbb{R}[\mathbf{X}]$.
% Let $\Sigma[\mathbf{X}]$ be the space of all sohs polynomials. 
 \end{definition}

The linear functional $L$ is nonnegative on $\mathbf{M}_{k}$. 
Given two polynomials $f,g\in\mathbb{R}[\mathbf{X}]$ and $f=\sum_{u} f_u u$, $g=\sum_{\nu} g_{\nu} \nu$.
Following the definition of the Hankel matrix $M_k$, we have that 
\begin{equation}
L(f^{\dag} g)=\sum_{u,\nu}f_u g_{\nu} L(u^{\dag}\nu)=\sum_{u,\nu}f_u g_{\nu} (M_k)_{u,\nu}=\mathbf{f}^T M_k\mathbf{g}.
\end{equation}
$f_i\in\mathbb{R}[\mathbf{x}]_d$ and $\mathbf{f}_i$ is the vector of coefficients.
Hence, it is easy to see that
\begin{equation}
M_k\succcurlyeq 0;\; M_{k_i}\succcurlyeq 0,\;\forall g_i\in\mathbf{g}.
\end{equation}

\begin{theorem}The dual problem $L_{\Theta_{2d}}(f,\mathbf{g})$ in Equation~\eqref{equ:trace-NCPO-dual} is an SDP.
\end{theorem}
\begin{proof}
We can transfer this problem to the space of Hankel matrix $M_d$.
We first look at the objective function of \eqref{equ:trace-NCPO-dual}.
Since $f\in\Sym\mathbb{R}[\mathbf{X}]_{2d}$, the polynomial $f$ can be expressed by a Gram matrix $G_f$, such that $f=\mathbf{W}^{\dag}_{k} G_f \mathbf{W}_{k}$ and $G_f$ is symmetric.
Using the proof of Lemma~\ref{lem:gram matrix}, we have
\begin{eqnarray*}
L(f)&=&L\left(\sum_{\omega\in \mathbf{W}_{2d}}f_{\omega}( \omega + \omega^{\dag})\right)\\
&=&\sum_{\omega\in \mathbf{W}_{2d}}f_{\omega} L( \omega + \omega^{\dag})\\
&=&\sum_{\omega\in \mathbf{W}_{2d}}f_{\omega}\left( L(u^{\dag}\nu) + L(\nu^{\dag} u)\right)\\
&=&\sum_{\omega\in \mathbf{W}_{2d}}f_{\omega}\left( \mathbf{u}^T M_d\mathbf{\nu} + \mathbf{\nu}^T M_d\mathbf{u}\right)\\
&=&\left\langle M_d,\sum_{\omega\in \mathbf{W}_{2d}}f_{\omega}\left(\mathbf{u}\mathbf{\nu}^T+\mathbf{\nu}\mathbf{u}^T\right)\right\rangle \\
&=& \langle M_d,G_p\rangle 
\end{eqnarray*}
Then, using Definition~\ref{defin:dual cones}, the first constraint $L\in\left(\Theta_{2d}\right)^{\vee}$ is a set of LMI . 
The last constraint $L(1)=1$ is equivalent to $\langle M_k, E_{1,1}\rangle=1$, where $E_{1,1}$ is a matrix with all entries 0 but $1$ in the $(1,1)$-entry. 
By reusing Definition~\ref{defin:dual cones}, we know that $L_{\Theta_{2d}}(f,\mathbf{g})$ is also an SDP.
\end{proof}

\begin{lemma}[\cite{helton2002positive}, Lemma~2.1]{}\label{lem:gram matrix}
For a polynomial $f\in\Sym\mathbb{R}[\mathbf{X}]_{2d}$, there exist a (non-unique) Gram matrix $G_f$, such that  
\begin{equation*}
f=W_{d}^{\dag}\; G_f\; W_{d},\; G^{\dag}_f=G_f,
\end{equation*}
where $W_{d}$ is a vector consisting all monomials in $\mathbf{W}_{d}$, which is introduced in Definition~\ref{def:monomial_basis_nc}.
\end{lemma}
\begin{proof}
A symmetric polynomial $f\in\Sym\mathbb{R}[\mathbf{X}]_{2d}$ is a weighted sum of symmetrised monomials, such that 
\begin{equation}
f=\sum_{\omega\in \mathbf{W}_{2d}}f_{\omega}( \omega + \omega^{\dag}),\label{equ:sum of symmetrized monomials}
\end{equation}
where $\omega\in \mathbf{W}_{2d}$ could be written as a product of two monomials
\begin{equation*}
\omega=u^{\dag} \nu,
\end{equation*}
with $u,\nu\in\mathbf{W}_d$. 
%\textcolor{red}{Recall from Section~\ref{app:GNS} that}
Let $\overrightarrow{f}$ denote the vector of coefficients of $f\in\mathbb{R}[\mathbf{X}]$.
Monomials $u,\nu$ could also be regarded as a polynomial, with
\begin{equation*}
u=\mathbf{u}^TW_d,\; \nu=\mathbf{\nu}^TW_d.
\end{equation*}
Since $\omega=\mathbf{W}^{\dag}_d \mathbf{u}\mathbf{\nu}^TW_d$ and $\omega^{\dag}=\mathbf{W}^{\dag}_d \mathbf{\nu}\mathbf{u}^TW_d$,
we show that the symmetrised monomial $\omega+\omega^{\dag}$ could be associated with a symmetric Gram matrix, such that 
\begin{equation}
\omega + \omega^{\dag}=W^{\dag}_d \left(\mathbf{u}\mathbf{\nu}^T+\mathbf{\nu}\mathbf{u}^T\right)W_d.
\label{equ:a symmetrized monomial}
\end{equation}
Substituting \eqref{equ:a symmetrized monomial} for \eqref{equ:sum of symmetrized monomials}, we then obtain a Gram matrix $G_f$ of $f$ as follows:
\begin{equation*}
G_f=\sum_{\omega\in \mathbf{W}_{2d}}p_{\omega}\left(\mathbf{u}\mathbf{\nu}^T+\mathbf{\nu}\mathbf{u}^T\right).
\end{equation*}
Using the fact that the weighted sum of symmetric matrices is also symmetric, we complete the proof.
\end{proof}


\section{Contributions of the Thesis}

After providing an overview of machine learning fairness, this thesis positions its contributions within the framework of enhancing fairness in machine learning, as outlined below.

\begin{itemize}
    \item \textbf{Proper Learning of Linear Dynamic Systems (Chapter~\ref{cha:tac}):}
        \begin{itemize}
            \item \textbf{Problem:} Identification of linear dynamic systems.
            \item \textbf{Innovation:} This method operates without assumptions about the dimensions of hidden dynamics, accommodating polynomial shape constraints with global optimality guarantees. The complexity can be mitigated through the exploitation of sparsity.
            \item \textbf{Methodology:} Non-Commutative Polynomial Problem (cf. Section~\ref{sec:ncpop}).
        \end{itemize}

    \item \textbf{Fairness in Forecasting from Imbalanced Data (Chapter~\ref{cha:jair}):}
        \begin{itemize}
            \item \textbf{Problem:} Imbalanced data (cf. Section~\ref{sec:imbalanced data}).
            \item \textbf{Innovation:} We present two fairness notions within the forecasting context. The global optimality proposed formulations rely on the technologies of non-commutative polynomial problem.
            \item \textbf{Methodology:} Proper Learning of Linear Dynamic Systems.
        \end{itemize}

    \item \textbf{Group-Blind Transport Map for Unavailable Sensitive Attributes (Chapter~\ref{cha:ot}):}
        \begin{itemize}
            \item \textbf{Problem:} Unavailability of sensitive attributes (cf. Section~\ref{sec:unvailable sa}).
            \item \textbf{Innovation:}
            We design a single group-blind projection map. The map aligns feature distributions of both majority and minority groups in source data, achieving demographic parity \citep{calder2009experimental} without requiring values of the protected attribute for individual samples in the computation or use of the map. 
            This contrasts with prevailing algorithms in fair learning, which rely predominantly on the accessibility or estimations of sensitive attributes, particularly during the training process.
            Instead, our approach utilises the feature distributions of the privileged and unprivileged groups in a boarder population and the essential assumption that the source data are unbiased representation of the population.
            \item \textbf{Methodology:} Dykstra's algorithm with Bregman projections \citep{bauschke2000dykstras}.
        \end{itemize}
\end{itemize}

\section{Structure of the Thesis}

\begin{itemize}
\item\textbf{Chapter~\ref{cha:introduction}: Introduction} 
\begin{itemize}
\item Introduce the state-of-the-art of machine learning fairness.
\item Outline the contributions of the thesis within this context.
\item Provide an overview of the thesis organisation.
\item Include a publication list.
\end{itemize}

\item\textbf{Chapters~\ref{cha:mom_app}-\ref{cha:jair}: Learning from Imbalanced Data} 
\begin{itemize}
\item Chapter 2: Discuss moment problems and their extension to non-commutative polynomial optimisation (NCPOP).
\item Chapter 3: Introduce the method for proper learning of linear dynamic systems, i.e., applying NCPOP to system identification.
\item Chapter 4: Present the method for fairness in forecasting from imbalanced data, i.e., applying proper learning of linear dynamic systems to fair learning.
\item Reference Section~\ref{sec:imbalanced data} for a discussion on imbalanced data.
\end{itemize}

\item\textbf{Chapter~\ref{cha:ot}: Learning with Unavailability of Sensitive Attributes} 
\begin{itemize}
\item Present the work for learning with the unavailability of sensitive attributes.
\item Reference Section~\ref{sec:unvailable sa} for a discussion on unavailable sensitive attributes.
\end{itemize}

\item\textbf{Appendix~\ref{app:notation}: Notation lists for Chapters 2-5}
\item\textbf{Appendix~\ref{app:sdp}:} Provide the fundamentals of semi-definite programming, serving as a preliminary for moment problems in Chapter 2.
\item\textbf{Appendix~\ref{app:ot}:} Include the proofs of all lemmas and theorems used in Chapter 5.
\end{itemize}


\section{Publication List}

\begin{itemize}
\item \bibentry{zhou2023learning}
\item \bibentry{zhou2023fairness}
\item \bibentry{zhou2023subgroup}
\item \bibentry{zhou2021fairness}
\end{itemize}


the world development report 2022 concerns that the recovery is going to be as uneven as its initial economic impacts.\footnote{See the world development report 2022 at \url{https://www.worldbank.org/en/publication/wdr2022}.} Disadvantaged populations and regions face a more prolonged journey towards recovering pandemic-induced losses of livelihoods, thereby exacerbating existing inequalities.

An article of International Monetary Fund 
(INEQUALITY IN THE TIME OF COVID-19) at \url{https://www.imf.org/external/pubs/ft/fandd/2021/06/inequality-and-covid-19-ferreira.htm}, states that the pandemic has also exacerbated preexisting inequalities in the labour market, largely because the ability to work remotely is highly correlated with education, and hence with pre-pandemic earnings. 
The stark reality is that job and income losses are likely to have hit lower-skilled and uneducated workers the hardest, 
when lower-skilled labor is predominantly informal, and those workers have no access to furlough programs or unemployment insurance. 

This year, hundreds of millions of such workers faced very stark trade-offs, on a daily basis, between staying safely at home or facing the threat of infection to provide food for their families.

In addition, with the burden of additional time required for childcare and housework falling disproportionately on women, gender inequality in earnings is particularly likely to have grown even wider.







In UK, 
In July 2020, Public Health England (PHE) (COVID-19: Review of disparities in risks and outcomes)
It confirms that the impact of COVID-19 has replicated existing health inequalities and, in some cases, has increased them. 
People of Black, Asian and other minority ethnic (BAME) groups were more exposed to COVID-19, more likely to be diagnosed with it and more likely to die from it. 

==> optimisation/intro-opt.tex <==


\chapter{The Challenge of Non-convex Optimisation}

Local optima and not necessarily global optima

Stationary points obtained by common heuristics only in some cases
% follow https://arxiv.org/abs/2001.07999

Undecidability of non-convex optimization

%  See the survey of https://www.lix.polytechnique.fr/~liberti/rairo18.pdf
% and explain:
%3.5.4 Unconstrained continuous global optimization . . . . . . . 11
%3.5.5 Box-constrained continuous global optimization . . . . . . . 12

NP-Hardness of polynomial optimization

% Explain
% https://www.sciencedirect.com/science/article/abs/pii/0167637788900491

General-purpose tools in non-convex optimization

%all have asymptotic convergence guarantees

Spatial branch and bound

Method of moments 

% here follow the blog post of Matteo? 
